Delta-Closure Structure for Studying Data Distribution

In this paper, we revisit pattern mining and study the distribution underlying a binary dataset thanks to the closure structure which is based on passkeys, i.e., minimum generators in equivalence classes robust to noise. We introduce $\Delta$-closedness, a generalization of the closure operator, where $\Delta$ measures how a closed set differs from its upper neighbors in the partial order induced by closure. A $\Delta$-class of equivalence includes minimum and maximum elements and allows us to characterize the distribution underlying the data. Moreover, the set of $\Delta$-classes of equivalence can be partitioned into the so-called $\Delta$-closure structure. In particular, a $\Delta$-class of equivalence with a high level demonstrates correlations among many attributes, which are supported by more observations when $\Delta$ is large. In the experiments, we study the $\Delta$-closure structure of several real-world datasets and show that this structure is very stable for large $\Delta$ and does not substantially depend on the data sampling used for the analysis.

==> 1234.tex <==
\centering
\setlength{\tabcolsep}{4pt}
\setlength\extrarowheight{5pt}
\begin{tabular}{lcccccc}
    $\mathcal{C}_1$&$a$&\begin{tabular}[c]{@{}c@{}}$abc$\\$\textcolor{gray}{(b)}$\end{tabular}&$c$&$d$&\begin{tabular}[c]{@{}c@{}}$ade$\\$\textcolor{gray}{(e)}$\end{tabular}&\begin{tabular}[c]{@{}c@{}}$abcdef$\\$\textcolor{gray}{f}$\end{tabular}\\ \hline
    $\mathcal{C}_2$& \multicolumn{2}{c}{$ac$} & \multicolumn{2}{c}{$ad$} & \multicolumn{2}{c}{$cd$} \\\hline 
    $\mathcal{C}_3$& \multicolumn{6}{c}{$acd$}
\end{tabular}

==> 1235.tex <==
\centering
\setlength{\tabcolsep}{4pt}
\setlength\extrarowheight{5pt}
\begin{tabular}{lcccccc}
    $\mathcal{C}_1$&$a$&$b$&\begin{tabular}[c]{@{}c@{}}$ac$\\\textcolor{gray}{$(c)$}\end{tabular}&$d$&\begin{tabular}[c]{@{}c@{}}$de$\\\textcolor{gray}{$(e)$}\end{tabular}&\begin{tabular}[c]{@{}c@{}}$bdef$\\$\textcolor{gray}{(f)}$\end{tabular}\\ \hline 
    $\mathcal{C}_2$&$ad$&\begin{tabular}[c]{@{}c@{}}$ade$\\$\textcolor{gray}{ae}$\end{tabular}&\begin{tabular}[c]{@{}c@{}}$acd$\\$\textcolor{gray}{cd}$\end{tabular}&\begin{tabular}[c]{@{}c@{}}$abc$\\$\textcolor{gray}{(ab,bc)}$\end{tabular} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}$abcdef$ \\$\textcolor{gray}{(af,ce,cf)}$\end{tabular}}
\end{tabular}

==> ME_F.tex <==
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l|ccc|c|cc|cc|c}\toprule
\multirow{2}{*}{name} & \multirow{2}{*}{$|G|$} & \multirow{2}{*}{$|M|$} & \multirow{2}{*}{\#attr.} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\#closed\\ itemsets\end{tabular}}& \multicolumn{2}{c}{\#nodes in $\mathcal{T}$} & \multicolumn{3}{c}{runtime, sec} \\
 &  &  &  &  & INT & EXT & INT & EXT & \begin{tabular}[c]{@{}c@{}}Charm +\\Talky-G\end{tabular}\\\midrule
adult & 48842 & 95 & 14 & 359141 & 359141 & 338906& 984 & 837 & 13\\
auto & 205 & 129 & 8 & 57789 & 57390 & 48834 & 6 & 2 & 5\\
breast & 699 & 14 & 10 & 361 & 361 & 354 & 0 & 0 & 1\\
car evaluation & 1728 & 21 & 6 & 8000 & 4875 & 6901 & 1 & 0 & 1\\
chess kr k & 28056 & 40 & 6 & 84636 & 54761 & 68869 & 146 & 148 & 5\\
cylinder bands & 540 & 120 & 39 & 39829537 & 39829537 & 37007525 & 2404 & 4010 & -$^\ast$\\
dermatology & 366 & 43 & 33 & 14152 & 10506 & 12172 & 1 & 1 & 1\\
ecoli & 327 & 24 & 8 & 425 & 425 & 373 & 0 & 0 & 1\\
glass & 214 & 40 & 10 & 3246 & 2393 & 2757 & 0 & 0 & 1\\
heart-disease & 303 & 45 & 0 & 25539 & 19388 & 21869 & 1 & 1 & 1\\
hepatitis & 155 & 50 & 19 & 144871 & 88039 & 122277 & 2 & 1 & 5\\
horse colic & 368 & 81 & 27 & 173866 & 138075 & 138075 & 11 & 9 & 10\\
ionosphere & 351 & 155 & 34 & 23202541 & 23202541 & 20354049 & 2467 & 2585 &12628 \\
iris & 150 & 16 & 4 & 120 & 80 & 111 & 0 & 0 & 1\\
led7 & 3200 & 14 & 7 & 1951 & 1012 & 1931 & 0 & 0 & 1\\
mushroom & 8124 & 88 & 22 & 181945 & 181945 & 171590 & 164 & 121 & 8\\
nursery & 12960 & 27 & 8 & 115200 & 76800 & 103351 & 46 & 51 & 4\\
page blocks & 5473 & 39 & 10 & 723 & 451 & 702 & 0 & 3 & 1\\
pen digits & 10992 & 76 & 16 & 3605507 & 2423123 & 3236109 & 12863 & 3398 & 123\\
pima & 768 & 36 & 0 & 1626 & 1105 & 1444 & 0 & 0 & 1\\
soybean & 683 & 99 & 35 & 2874252 & 2726204 & 2640461 & 379 & 224 & 298\\
tic tac toe & 958 & 27 & 9 & 42712 & 25276 & 34513 & 1 & 1 & 1\\
wine & 178 & 65 & 13 & 13229 & 8518 & 10202 & 1 & 1 &  2 \\
zoo & 101 & 35 & 17 & 4570 & 2933 & 4125 & 0 & 0 &  1\\\midrule
\textbf{average} & 5239 & 57 & 15 & 2947747 & 2883953 & 2680313 & 812 & 475 & 376\\\toprule
\end{tabular}\\
\begin{flushleft}
$^\ast$ The algorithm crashes because of the lack of memory.
\end{flushleft}


==> algos.tex <==
%\begin{minipage}[t]{.5\textwidth}
%    \begin{algorithm}[H]
%    \caption{GDPM-ME}
%    \label{alg:gdpm_me}
%    \begin{algorithmic}[1]
%        \REQUIRE $\mathcal{C}_{k-1}$, formal concepts of the level $k-1$,\\
%        $\mathcal{T}_{k-1}$, the trie containing all closed itemsets $\bigcup_{i = 1, \ldots, k-1}\{B \mid %(A,B) \in \mathcal{C}_i\}$
%        \ENSURE $\mathcal{C}_{k}$, formal concepts of the level $k$
%        \STATE  $\mathcal{C}_{k} \leftarrow \emptyset $
%        \STATE  $\mathcal{T}_{k} \leftarrow \mathcal{T}_{k-1}$
%        \FORALL{$(A,B) \in \mathcal{C}_{k-1}$}
%            \FORALL{$m \in M \setminus B$}\label{line:candidates}
%                \STATE $A^\ast = \{g \mid (g,m) \in I, g \in A\}$\label{line:me_A}
%                \IF{$|A^\ast| > 0$}
%                    \STATE $B^\ast = \{ m^\ast \mid (g,m^\ast) \in I, m^\ast \in  M, g \in  %A^\ast\}$\label{line:me_B}
%                    \IF{$B^\ast \notin \mathcal{T}_{k}$}\label{line:me_tree_check}
%                        \STATE $add(\mathcal{T}_{k},B^\ast)$ 
%                        \STATE $add(\mathcal{C}_{k},(A^\ast,B^\ast))$ 
%                    \ENDIF	
%                \ENDIF
%            \ENDFOR
%        \ENDFOR
%        \RETURN $\mathcal{C}_{k}$
%    \end{algorithmic}
%    \end{algorithm}
%\end{minipage}
%\begin{minipage}[t]{.48\textwidth}   
%    \begin{algorithm}[H]
%    \caption{GDPM-F}
%    \label{alg:gdpm_f}
%    \begin{algorithmic}[1]
%        \REQUIRE $\mathcal{C}_{k-1}$, formal concepts of the level $k-1$,\\
%        $\mathcal{T}_{k-1}$, the trie containing all extents $\bigcup_{i = 1, \ldots, k-1}\{A \mid (A,B) %\in \mathcal{C}_i\}$
%        \ENSURE $\mathcal{C}_{k}$, formal concepts of the level $k$
%        \STATE  $\mathcal{C}_{k} \leftarrow \emptyset $
%        \STATE  $\mathcal{T}_{k} \leftarrow \mathcal{T}_{k-1}$
%        \FORALL{$(A,B) \in \mathcal{C}_{k-1}$}
%            \FORALL{$m \in M \setminus B$}
%                \STATE $A^\ast = \{g \mid (g,m) \in I, g \in A\}$ \label{line:f_A}
%                \IF{$|A^\ast|\notin \mathcal{T}_{k}$} \label{line:f_tree_check}
%                    \STATE $B^\ast = \{ m^\ast \mid (g,m^\ast) \in I, m^\ast \in  M, g \in  A^\ast\}$ %\label{line:f_B}
%                    \STATE $add(\mathcal{T}_{k},A\ast)$ 
%                    \STATE $add(\mathcal{C}_{k},(A^\ast,B^\ast))$ 
%                \ENDIF
%            \ENDFOR
%        \ENDFOR
%        \RETURN $\mathcal{C}_{k}$
%    \end{algorithmic}
%    \end{algorithm}
%\end{minipage}

%    \begin{algorithm}[H]
%    \caption{GDPM-INT//GDPM-EXT}
%    \label{alg:gdpm_me}
%    \begin{algorithmic}[1]
%        \REQUIRE $\mathcal{C}_{k-1}$, formal concepts of the level %$k-1$,\\
%        $\mathcal{T}_{k-1}$, the trie containing all closed %itemsets $\bigcup_{i = 1, \ldots, k-1}\{B \mid (A,B) \in %\mathcal{C}_i\}$ (ME) // their extents $\bigcup_{i = 1, %\ldots, k-1}\{A \mid (A,B) \in \mathcal{C}\}$ (F)
%        \ENSURE $\mathcal{C}_{k}$, formal concepts of the level %$k$
%        \STATE  $\mathcal{C}_{k} \leftarrow \emptyset $
%        \STATE  $\mathcal{T}_{k} \leftarrow \mathcal{T}_{k-1}$
%        \FORALL{$(A,B) \in \mathcal{C}_{k-1}$}
%            \FORALL{$m \in M \setminus B$}\label{line:candidates}
%                \STATE $A^\ast = \{g \mid (g,m) \in I, g \in %A\}$\label{line:me_A}
%                \IF{$|A^\ast| > 0$ \textbf{ then } // \textbf{ if %}{$|A^\ast|\notin %\mathcal{T}_{k}$}}\label{line:f_tree_check} 
%                    \STATE $B^\ast = \{ m^\ast \mid (g,m^\ast) \in %I, m^\ast \in  M, g \in  %A^\ast\}$\label{line:me_B}
%                    \IF{$B^\ast \notin \mathcal{T}_{k}$ \textbf{ %then } // \textbf{ no if %-}}\label{line:me_tree_check}
%                        \STATE $add(\mathcal{T}_{k},B^\ast)$  // %$add(\mathcal{T}_{k},A^\ast)$\label{line:a%dd_to_tree} 
%                        \STATE %$add(\mathcal{C}_{k},(A^\ast,B^\ast))$ 
%                    \ENDIF	
%                \ENDIF
%            \ENDFOR
%        \ENDFOR
%        \RETURN $\mathcal{C}_{k}$  
%    \end{algorithmic}
%    \end{algorithm}
    
    
\begin{algorithm}[H]
    \caption{GDPM-INT\hspace{3.em} // GDPM-EXT}
    \label{alg:gdpm_int}
    \begin{algorithmic}[1]
        \REQUIRE $\mathcal{C}_{k-1}$, closed itemsets of the level $k-1$,\\
        $\mathcal{T}_{k-1}$, the trie containing all closed itemsets $\bigcup_{i = 1, \ldots, k-1}\{B \mid B \in \mathcal{C}_i\}$ 
        \ENSURE $\mathcal{C}_{k}$, closed itemsets of the level $k$
        \STATE  $\mathcal{C}_{k} \leftarrow \emptyset $
        \STATE  $\mathcal{T}_{k} \leftarrow \mathcal{T}_{k-1}$
        \FORALL{$B \in \mathcal{C}_{k-1}$}
            \FORALL{$m \in M \setminus B$}\label{line:candidates} 
                \STATE $B_c \leftarrow (B \cup \{m\})''$\label{line:closure}  \hspace{4.2em}  // $A_c \leftarrow (B \cup \{m\})'$
                    \IF{$B_c \notin \mathcal{T}_{k} \textbf{ then  }  \hspace{5em} //\textbf{  if }A_c \notin \mathcal{T}_{k}$}\label{line:tree_check} 
                        \STATE $add(\mathcal{T}_{k},B_c)$\label{line:add_to_tree}  \hspace{5.5em}   // \hspace{1.5em} $add(\mathcal{T}_{k},A_c)$
                        \STATE $add(\mathcal{C}_{k},B_c)$\label{line:add_to_cl}  \hspace{5.4em}   // \hspace{1.5em}  $add(\mathcal{C}_{k},A_c')$
                    \ENDIF	
            \ENDFOR
        \ENDFOR
        \RETURN $\mathcal{C}_{k}$  
    \end{algorithmic}
    \end{algorithm}

==> bma_levels.tex <==
%\rotatebox{90}{
\setlength{\tabcolsep}{4pt}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{l|l|cccccccccccccccc}\toprule
 &  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\ \midrule
\multirow{2}{*}{1} & count &{\color[HTML]{9B9B9B}163}&  &  &  & 1 &  &  &  &  &  &  &  &  &  &  &  \\
 &sup.&{\color[HTML]{9B9B9B}211.4+304.1}&  &  &  & 2.0+0.0 &  &  &  &  &  &  &  &  &  &  &  \\\hline
\multirow{2}{*}{2} & count &  &{\color[HTML]{9B9B9B}5637}& 629 & 264& 136& 71& 26 & 17 & 14 & 3 & 2 & 1& 1 & 1 &  &  \\
 &sup.&  &{\color[HTML]{9B9B9B}18.3+31.6}& 2.8+1.1 & 2.3+0.6 & 2.1+0.3 & 2.1+0.4 & 2.1+0.4 & 2.1+0.2 & 2.0+0.0 & 2.0+0.0 & 2.0+0.0 & 2.0+0.0 & 2.0+0.0 & 2.0+0.0 &  &  \\\hline
\multirow{2}{*}{3} & count &  &  &{\color[HTML]{9B9B9B}27051}& 7655& 3409& 1483 & 677& 294 & 108 & 57 & 21 & 8 & 3 & 3 & 1 & 1 \\
 &sup.&  &  &{\color[HTML]{9B9B9B}6.8+7.7}& 2.8+1.1 & 2.4+0.7 & 2.2+0.5 & 2.1+0.4 & 2.1+0.3 & 2.1+0.2 & 2.1+0.3 & 2.0+0.0 & 2.0+0.0 & 2.0+0.0 & 2.0+0.0 & 2.0+0.0 & 2.0+0.0 \\\hline
\multirow{2}{*}{4} & count &  &  &  &{\color[HTML]{9B9B9B}28841}& 10115& 3526& 1211 & 376& 84 & 24 & 6 & 1 &  &  &  &  \\
 &sup.&  &  &  &{\color[HTML]{9B9B9B}4.6+3.3}& 2.9+1.1 & 2.5+0.8 & 2.3+0.6 & 2.2+0.4 & 2.1+0.3 & 2.1+0.3 & 2.0+0.0 & 2.0+0.0 &  &  &  &  \\\hline
\multirow{2}{*}{5} & count &  &  &  &  &{\color[HTML]{9B9B9B}7681}& 2258 & 463& 96 & 14 &  &  &  &  &  &  &  \\
 &sup.&  &  &  &  &{\color[HTML]{9B9B9B}4.0+2.1}& 3.0+1.2 & 2.6+0.8 & 2.3+0.6 & 2.2+0.4 &  &  &  &  &  &  &  \\\hline
\multirow{2}{*}{6} & count &  &  &  &  &  &{\color[HTML]{9B9B9B}504}& 106& 7&  &  &  &  &  &  &  &  \\
 &sup.&  &  &  &  &  &{\color[HTML]{9B9B9B}3.7+1.6}& 3.1+0.9 & 2.7+0.7 &  &  &  &  &  &  &  &  \\\hline
\multirow{2}{*}{7} & count &  &  &  &  &  &  &{\color[HTML]{9B9B9B}3}&  &  &  &  &  &  &  &  &  \\
 &sup.&  &  &  &  &  &  &{\color[HTML]{9B9B9B}4.3+0.5}&  &  &  &  &  &  &  &  & \\\bottomrule
\end{tabular}
}
%}

==> clst_key.tex <==
\centering
\setlength{\tabcolsep}{4pt}
\setlength\extrarowheight{5pt}
\begin{tabular}{lcccccccccc}
$\mathcal{C}_1$&$a$&$b$&$c$&$d$&$e$&{\begin{tabular}[c]{@{}c@{}}$bef$\\$\textcolor{gray}{(f)}$\end{tabular}}&& & \\ \hline% \\ \hline \\
$\mathcal{C}_2$& \begin{tabular}[c]{@{}c@{}}$abc$\\$\textcolor{gray}{(ab,bc)}$\end{tabular}& \begin{tabular}[c]{@{}c@{}}$bdef$\\$\textcolor{gray}{(bd,df)}$\end{tabular} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}$abcdef$\\$\textcolor{gray}{(af,cf,ce)}$\end{tabular}}&\begin{tabular}[c]{@{}c@{}}$ade$\\$\textcolor{gray}{(ae)}$\end{tabular}& \begin{tabular}[c]{@{}c@{}}$bef$\\$\textcolor{gray}{(be)}$\end{tabular} &$ac$&$de$&$ad$&$cd$\\ \hline%\\ \hline \\
$\mathcal{C}_3$&$acd$&\multicolumn{5}{c}{\begin{tabular}[c]{@{}c@{}}$abcdef$\\$\textcolor{gray}{(abd, abe, bcd)}$\end{tabular}}
\end{tabular}


==> clst_mkey.tex <==
\centering
\setlength{\tabcolsep}{4pt}
%\setlength\extrarowheight{5pt}
\begin{tabular}{lcccccccccc}
$\mathcal{C}_0$ & $\bm{\emptyset}$\\\hline
$\mathcal{C}_1$&$\bm{a}$&$\bm{b}$&$ab\bm{c}$&$ab\bm{d}$&$ab\bm{e}$&$abc\bm{f}$&$abc\bm{g}$&$abde\bm{h}$&$abde\bm{i}$&\\ \hline% \\ \hline \\
$\mathcal{C}_2$&$\bm{ab}$&$ab\bm{cd}$&$ab\bm{ce}$&$ab\bm{de}$& \multicolumn{4}{c}{$abcd\bm{ef}ghi$ $(\bm{eg}, \bm{fg}, \bm{fh}, \bm{fi}, \bm{gh}, \bm{gi}, \bm{hi})$}\\ \hline%\\ \hline \\
$\mathcal{C}_3$&$abcde$&\\
\end{tabular}


==> data_description.tex <==
%\begin{tabular}{l|ccccccr}
%    \toprule
%    name &$|G|$&$|M|$& density & \#classes &\#attributes& $N_c^{min}$ & \#concepts \\
%    \midrule
%    adult & 48842 & 95 & 0.15 & 2 & 14 & 12 & 359141 \\
%    auto & 205 & 129 & 0.19 & 6 & 8 & 8 & 57789.0 \\
%    breast & 699 & 14 & 0.64 & 2 & 10 & 6 & 361 \\
%    car\_evaluation & 1728 & 21 & 0.29 & 4 & 6 & 6 & 8000 \\
%    chess\_kr\_k & 28056 & 40 & 0.15 & 18 & 6 & 6 & 84636 \\
%    cylinder\_bands & 540 & 120 & 0.28 & 2 & 39 & 19 & 39829537 \\
%    dermatology & 366 & 43 & 0.28 & 6 & 33 & 9 & 14152 \\
%    ecoli & 327 & 24 & 0.29 & 5 & 8 & 6 & 425 \\
%    glass & 214 & 40 & 0.22 & 6 & 10 & 8 & 3246 \\
%    heart-disease & 303 & 45 & 0.29 & 5 & 0 & 9 & 25539 \\
%    hepatitis & 155 & 50 & 0.36 & 2 & 19 & 11 & 144871 \\
%    horse\_colic & 368 & 81 & 0.21 & 2 & 27 & 9 & 173866 \\
%    iris & 150 & 16 & 0.25 & 3 & 4 & 4 & 120.0 \\
%    led7 & 3200 & 14 & 0.5 & 10 & 7 & 7 & 1951.0 \\
%    mushroom & 8124 & 88 & 0.25 & 2 & 22 & 10 & 181945 \\
%    nursery & 12960 & 27 & 0.3 & 5 & 8 & 8 & 115200 \\
%    page\_blocks & 5473 & 39 & 0.26 & 5 & 10 & 8 & 723 \\
%    pen\_digits & 10992 & 76 & 0.21 & 10 & 16 & 11 & 3605507 \\
%    pima & 768 & 36 & 0.22 & 2 & 0 & 8 & 1626 \\
%    soybean & 683 & 99 & 0.32 & 19 & 35 & 13 & 2874252 \\
%    tic\_tac\_toe & 958 & 27 & 0.33 & 2 & 9 & 7 & 42712 \\
%    wine & 178 & 65 & 0.2 & 3 & 13 & 7 & 13229 \\
%    zoo & 101 & 35 & 0.46 & 7 & 17 & 7 & 4570\\
%    \bottomrule
%\end{tabular}
\setlength{\tabcolsep}{2.1pt}
\begin{tabular}{l|cccccc|l} \toprule
name &$|G|$&$|M|$&density&\#classes&\#attr.&\begin{tabular}[c]{@{}c@{}}closure\\index\\$CI$\end{tabular}& $2^{CI} \leq |\mathcal{C}| \leq 2^{\min(|M|,|G|)}$ \\\midrule
adult & 48842 & 95 & 0.15 & 2 & 14 & 12 &4.1e+3 $\leq$ 3.6e+5 $\leq$ 4.0e+28 \\
auto & 205 & 129 & 0.19 & 6 &\underline{\textbf{8}}&\underline{\textbf{8}}& 2.6e+2 $\leq$ 5.8e+4 $\leq$ 6.8e+38 \\
breast & 699 & 14 & 0.64 & 2 & 10 & 6 & 6.4e+1 $\leq$ 3.6e+2 $\leq$ 1.6e+4 \\
car evaluation & 1728 & 21 & 0.29 & 4 &\underline{\textbf{6}}&\underline{\textbf{6}}& 6.4e+1 $\leq$ 8.0e+3 $\leq$ 2.1e+6 \\
chess kr k & 28056 & 40 & 0.15 & 18 &\underline{\textbf{6}}&\underline{\textbf{6}}& 6.4e+1 $\leq$ 8.5e+4 $\leq$ 1.1e+12 \\
cylinder bands & 540 & 120 & 0.28 & 2 & 39 & 19 & 5.2e+5 $\leq$ 4.0e+7 $\leq$ 1.3e+36 \\
dermatology & 366 & 43 & 0.28 & 6 & 33 & 9 & 5.1e+2 $\leq$ 1.4e+4 $\leq$ 8.8e+12 \\
ecoli & 327 & 24 & 0.29 & 5 & 8 & 6 & 6.4e+1 $\leq$ 4.3e+2 $\leq$ 1.7e+7 \\
glass & 214 & 40 & 0.22 & 6 & 10 & 8 & 2.6e+2 $\leq$ 3.2e+3 $\leq$ 1.1e+12 \\
heart-disease & 303 & 45 & 0.29 & 5 &  & 9 & 5.1e+2 $\leq$ 2.6e+4 $\leq$ 3.5e+13 \\
hepatitis & 155 & 50 & 0.36 & 2 & 19 & 11 & 2.0e+3 $\leq$ 1.4e+5 $\leq$ 1.1e+15 \\
horse colic & 368 & 81 & 0.21 & 2 & 27 & 9 & 5.1e+2 $\leq$ 1.7e+5 $\leq$ 2.4e+24 \\
ionosphere & 351 & 155 & 0.22 & 2 & 34 & 17 & 1.3e+5 $\leq$ 2.3e+7 $\leq$ 4.6e+46 \\
iris & 150 & 16 & 0.25 & 3 &\underline{\textbf{4}}&\underline{\textbf{4}}& 1.6e+1 $\leq$ 1.2e+2 $\leq$ 6.6e+4 \\
led7 & 3200 & 14 & 0.50 & 10 &\underline{\textbf{7}}&\underline{\textbf{7}}& 1.3e+2 $\leq$ 2.0e+3 $\leq$ 1.6e+4 \\
mushroom & 8124 & 88 & 0.25 & 2 & 22 & 10 & 1.0e+3 $\leq$ 1.8e+5 $\leq$ 3.1e+26 \\
nursery & 12960 & 27 & 0.30 & 5 &\underline{\textbf{8}}&\underline{\textbf{8}}& 2.6e+2 $\leq$ 1.2e+5 $\leq$ 1.3e+8 \\
page blocks & 5473 & 39 & 0.26 & 5 & 10 & 8 & 2.6e+2 $\leq$ 7.2e+2 $\leq$ 5.5e+11 \\
pen digits & 10992 & 76 & 0.21 & 10 & 16 & 11 & 2.0e+3 $\leq$ 3.6e+6 $\leq$ 7.6e+22 \\
pima & 768 & 36 & 0.22 & 2 & & 8 & 2.6e+2 $\leq$ 1.6e+3 $\leq$ 6.9e+10 \\
soybean & 683 & 99 & 0.32 & 19 & 35 & 13 & 8.2e+3 $\leq$ 2.9e+6 $\leq$ 6.3e+29 \\
tic tac toe & 958 & 27 & 0.33 & 2 & 9 & 7 & 1.3e+2 $\leq$ 4.3e+4 $\leq$ 1.3e+8 \\
wine & 178 & 65 & 0.20 & 3 & 13 & 7 & 1.3e+2 $\leq$ 1.3e+4 $\leq$ 3.7e+19 \\
zoo & 101 & 35 & 0.46 & 7 & 17 & 7 & 1.3e+2 $\leq$ 4.6e+3 $\leq$ 3.4e+10 \\\bottomrule
\end{tabular}

==> keys_min_keys.tex <==
\centering
\setlength{\tabcolsep}{4pt}
\setlength\extrarowheight{5pt}
\begin{tabular}{lcccc}
    $\mathcal{C}_1$&$a$&$b$&$c$& \begin{tabular}[c]{@{}c@{}}$abcd$\\$\textcolor{gray}{(d)}$\end{tabular} \\ \hline 
    $\mathcal{C}_2$&$ab$&$bc$&$ac$&  %\\  \hline 
%    $\mathcal{C}_3$& \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}$abcd$\\$\textcolor{gray}{(abc)}$\end{tabular}} & 
\end{tabular}

==> name.tex <==
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{d_pk_adult.png}
        \caption{``adult''}
        \label{fig:d_pk_adult}
    \end{subfigure}
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{d_pk_chess_kr_k.png}
        \caption{``chess kr k''}
        \label{fig:d_pk_chess_kr_k}
    \end{subfigure}
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{d_pk_car_evaluation.png}
        \caption{``car evaluation''}
        \label{fig:d_pk_car}
    \end{subfigure}
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{d_pk_pima.png}
        \caption{``pima''}
        \label{fig:d_pk_pima}
    \end{subfigure}
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{d_pk_auto.png}
        \caption{``auto''}
        \label{fig:d_pk_auto}
    \end{subfigure}
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{d_pk_led7.png}
        \caption{``led7''}
        \label{fig:d_pk_led7}
    \end{subfigure}
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{d_pk_nursery.png}
        \caption{``nursery''}
        \label{fig:d_pk_nursery}
    \end{subfigure}   
    \begin{subfigure}{0.3\columnwidth}
        \includegraphics[width=\textwidth]{d_pk_page_blocks.png}
        \caption{``page blocks''}
        \label{fig:d_pk_page_blocks}
    \end{subfigure}
    \caption{The distribution of \textDelta-passkeys by levels}
    \label{fig:delta}

==> new-sample-123456.tex <==
%\centering
%\setlength{\tabcolsep}{4pt}
%\setlength\extrarowheight{5pt}
\begin{tabular}[t]{lc}
    $\mathcal{C}_0$& \clsPK{abc}{\emptyset} \\
    \hline
    %$\mathcal{C}_1$& \clsPK{abcd}{d}\hfill\clsPK{abce}{e}\hfill\clsPK{abcf}{f}\hfill\clsPK{abcg}{g}\hfill\clsPK{M}{i}\\
    $\mathcal{C}_1$& $abc\bm{d}$ \hfill $abc\bm{e}$ \hfill $abc\bm{f}$ \hfill $abc\bm{g}$ \hfill \clsPK{M}{i}\\
    \hline
    %$\mathcal{C}_2$& \clsPK{abcde}{de} \\
    $\mathcal{C}_2$& $abc\bm{de}$ \\
    \hline
    %$\mathcal{C}_3$ & --- \\
    $\mathcal{C}_3$ & --- \\
\end{tabular}

==> new-sample-123478.tex <==
%\centering
%\setlength{\tabcolsep}{4pt}
%\setlength\extrarowheight{5pt}
\begin{tabular}[t]{lc}
    $\mathcal{C}_0$& \clsPK{ab}{\emptyset} \\
    \hline
    %$\mathcal{C}_1$& \clsPK{abc}{c}\hfill\clsPK{abd}{d}\hfill\clsPK{abe}{e} \hfill \clsPK{abch}{h} \hfill \clsPK{abci}{i} \hfill \clsPK{M}{f}\\
    $\mathcal{C}_1$& $ab\bm{c}$ \hfill $ab\bm{d}$ \hfill $ab\bm{e}$ \hfill $abc\bm{h}$ \hfill $abc\bm{i}$ \hfill \clsPK{M}{f}\\
    \hline
    %$\mathcal{C}_2$& \clsPK{abcd}{cd}\hfill\clsPK{abce}{ce}\hfill\clsPK{abde}{de}  \\
    $\mathcal{C}_2$& $ab\bm{cd}$ \hfill $ab\bm{ce}$ \hfill $ab\bm{de}$ \\
    \hline
    %$\mathcal{C}_3$& \clsPK{abcde}{cde}\\
    $\mathcal{C}_3$& $ab\bm{cde}$\\
\end{tabular}

==> rules_by_conf_0005.tex <==
\setlength{\tabcolsep}{2pt}    
\begin{tabular}{L{4.5cm}L{4.5cm}|c|c|c} \toprule
    antecedents & consequents &support&conf&lift\\ \midrule
    \nt{`frankfurter', `frozen fish',\\`whole milk', `pip fruit'}&`frozen meals', `other vegetables', `yogurt', `tropical fruit'&0.0005&1&1567.0\\\hline
    `grapes', `frozen fish'&`frozen meals', `pip fruit', `other vegetables',`tropical fruit', `whole milk'&0.0005&1&1119.3\\\hline
    \nt{`frozen meals', `other vegetables',\\`yogurt', `frankfurter'}&\nt{`tropical fruit', `frozen fish',\\ `whole milk', `pip fruit'}&0.0005&1&1119.3\\\hline
    `grapes', `frozen fish'&\nt{`frozen meals', `other vegetables',\\`tropical fruit', `pip fruit'}&0.0005&1&870.6\\\hline
    `grapes', `whole milk', `frozen fish'&\nt{`frozen meals', `other vegetables',\\`tropical fruit', `pip fruit'}&0.0005&1&870.6\\\bottomrule
%    'grapes', 'frozen fish'&\nt{'frozen meals', 'other vegetables',\\'whole milk', 'pip fruit'}&783.5\\
%    \nt{'frozen meals', 'other vegetables',\\'yogurt', 'frankfurter'}&\nt{'tropical fruit', 'frozen fish',\\ 'pip fruit'}&783.5\\
%    'tropical fruit', 'grapes', 'frozen fish'&\nt{'frozen meals', 'other vegetables',\\'whole milk', 'pip fruit'}&783.5\\
%    \nt{'frozen meals', 'yogurt', \\'pip fruit', 'other vegetables',\\'tropical fruit'}&\nt{'frankfurter', 'whole milk',\\'frozen fish'}&783.5\\
%    \nt{'frozen meals', 'yogurt', \\'other vegetables', 'frankfurter',\\'whole milk'}&\nt{'tropical fruit', 'frozen fish',\\'pip fruit'}&783.5\\
%    \nt{'domestic eggs', 'citrus fruit',\\'misc. beverages'}&'whole milk', 'canned fruit'&712.3\\
%    \nt{'frozen meals', 'other vegetables',\\'yogurt', 'frankfurter'}&\nt{'frozen fish', 'whole milk',\\'pip fruit'}&712.3\\
%    \nt{'frozen meals', 'yogurt',\\'other vegetables', 'tropical fruit',\\'frankfurter'}&\nt{'frozen fish', 'whole milk',\\'pip fruit'}&712.3\\
%    \nt{'frozen meals', 'yogurt',\\'whole milk', 'frozen fish'}&\nt{'other vegetables', 'tropical fruit',\\ 'frankfurter', 'pip fruit'}&712.3\\\bottomrule
    \end{tabular}
